Multi-Step Visual Reasoning with Visual Tokens Scaling and Verification

Multi-modal large language models (MLLMs) have achieved remarkable capabilities by integrating visual perception with language understanding, enabling applications such as image-grounded dialogue, visual question answering, and scientific analysis. However, most MLLMs adopt a static inference paradigm, encoding the entire image into fixed visual tokens upfront, which limits their ability to iteratively refine understanding or adapt to context during inference. This contrasts sharply with human perception, which is dynamic, selective, and feedback-driven. In this work, we introduce a novel framework for inference-time visual token scaling that enables MLLMs to perform iterative, verifier-guided reasoning over visual content. We formulate the problem as a Markov Decision Process, involving a reasoner that proposes visual actions and a verifier, which is trained via multi-step Direct Preference Optimization (DPO), that evaluates these actions and determines when reasoning should terminate. To support this, we present a new dataset, VTS, comprising supervised reasoning trajectories (VTS-SFT) and preference-labeled reasoning comparisons (VTS-DPO). Our method significantly outperforms existing approaches across diverse visual reasoning benchmarks, offering not only improved accuracy but also more interpretable and grounded reasoning processes. These results demonstrate the promise of dynamic inference mechanisms for enabling fine-grained, context-aware visual reasoning in next-generation MLLMs.

==> tables/data_statistics.tex <==
\begin{longtable}{@{\extracolsep{\fill}}llrrrrrr@{}}
\scriptsize
\centering
\caption{Dataset Statistics} \label{tab:dataset_stats} 
\toprule
\multirow{2}{*}{Subset} & \multirow{2}{*}{Instance \#} & \multicolumn{2}{r}{All Sampled \#} & \multicolumn{2}{r}{DPO Dataset \#} & \multicolumn{2}{r}{SFT Dataset\#} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
 & & Count & Pct. & Count & Pct. & Count & Pct. \\
\midrule
\endfirsthead % 表头在第一页显示
\multicolumn{8}{c}{Dataset Statistics} \\
\toprule
\multirow{2}{*}{Subset} & \multirow{2}{*}{Instance \#} & \multicolumn{2}{r}{All Sampled \#} & \multicolumn{2}{r}{DPO Dataset \#} & \multicolumn{2}{r}{SFT Dataset\#} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
 & & Count & Pct. & Count & Pct. & Count & Pct. \\
\midrule
\endhead % 表头在后续页重复
\bottomrule
\endfoot % 表尾在每页底部
\endlastfoot % 表尾在最后一页底部
ai2d(cauldron,llava\_format) & 2,429 & 657& 27.0& 641 & 26.4 & 585 & 24.1 \\
ai2d(gpt4v) & 4,864 & 1,454& 29.9& 1105 & 22.7 & 1,101 & 22.6 \\
allava\_instruct\_laion4v  & 49,990 & 15,729 & 31.5& 9640 & 19.3 & 9,225 & 18.5 \\
allava\_instruct\_vflan4v  & 19,990 & 4,965 & 24.8& 2,906 & 14.5 & 2,853 & 14.3 \\
aokvqa(cauldron,llava\_format)  & 16,534  & 3,578 & 21.6& 2,007 & 12.1 & 2,013 & 12.2 \\
ai2d(internvl)  & 12,403  & 2,027 & 16.3& 1,694 & 13.7 & 1,317 & 10.6 \\
CLEVR-Math(MathV360K)  & 5,280  & 5,227 & 99.0& 2,761 & 52.3 & 2,827 & 53.5 \\
chart2text(cauldron)  & 26,956  & 9,825 & 36.4& 3,053 & 11.3 & 3,647 & 13.5 \\
clevr(cauldron,llava\_format)  & 69,995  & 20,973 & 30.0& 16,746 & 23.9 & 16,915 & 24.2 \\
chartqa(cauldron,llava\_format)  & 18,260  & 5,455 & 29.9& 4,084 & 22.4 & 3,034 & 16.6 \\
chrome\_writting & 8,825  & 2,280 & 25.8& 1,591 & 18.0 & 1,543 & 17.5 \\

dvqa(cauldron,llava\_format) & 199,995  & 59,923 & 30.0& 32,443 & 16.2 & 42,568 & 21.3 \\
diagram\_image\_to\_text(cauldron) & 295  & 85 & 28.8& 67 & 22.7 & 66 & 22.4 \\
FigureQA(MathV360K)  & 17,587  & 17,569  & 99.9& 9,121 & 51.9 & 7,309 & 41.6 \\
figureqa(cauldron,llava\_format)  & 99,995  & 29,203  & 29.2& 27,762 & 27.8 & 23,050 & 23.1 \\
GEOS(MathV360K) & 498  & 494  & 99.2& 201 & 40.4 & 111 & 22.3 \\
GeoQA+(MathV360K) & 17,162  & 6,759  & 39.4& - & - & 1,852 & 10.8 \\
geo3k & 2,091  & 625  & 29.9& 463 & 22.1 & 182 & 8.7 \\
geomverse(cauldron) & 9,298  & 2,524 & 27.1 & 1,030 & 11.1 & 749 & 8.1 \\
Geometry3K(MathV360K) & 9,724  & 2,287 & 23.5 & 970 & 10.0 &519  &5.3 \\
geo170k(align) & 60,242  & 5,558 & 9.2 & 467 & 0.8 &475 & 0.8 \\
geo170k(qa) & 67,823  & 5,612 & 8.3 & 2,975 & 4.4 & 1,136 & 1.7\\
hateful\_memes(cauldron,llava\_format)  & 8,495  & 2,481 & 29.2 & 1,775 & 20.9 & 1,707 & 20.1 \\
hme100k & 74,492  & 11,790 & 15.8& 7,193 & 9.7 & 7,290 & 9.8 \\
hitab(cauldron,llava\_format)  & 2,495  & 372 & 14.9& 274 & 11.0 & 256 & 10.3 \\
infographic\_vqa\_llava\_format & 2,113  & 2,097 & 99.2& 1,532 & 72.5 & 1,579  & 74.7 \\
intergps(cauldron,llava\_format) & 1,275  & 762 & 59.8 & 187 & 14.7 & 85 & 6.7 \\
image\_textualization(filtered) & 99,573  & 29,816 & 29.9 & 4,422 & 4.4 & 3,431 & 3.4\\
iam(cauldron) & 5,658  & 1,670 & 29.5 & - & - & 1,339 & 23.7 \\
infographic\_vqa  & 4,394  & 1,207 & 27.5 & 987 & 22.5 & 961 & 21.9 \\
infographic(gpt4v)  & 1,982  & 500 & 25.2 & 386 & 19.5 & 246 & 12.4 \\
iconqa(cauldron,llava\_format)  & 27,302  & 6,609 & 24.2 & 5,424  & 19.9 & 4,226 & 15.5 \\
IconQA(MathV360K)  & 22,589  & 5,036 & 22.3 & 3,031 & 13.4 & 1,886 & 8.3 \\
iiit5k & 1,990  & 324 & 16.3 & 290  & 14.6 & 297  & 14.9 \\
k12\_printing & 256,636  & 320 & 0.1 & 179 & 0.1 & 211  & 0.1 \\
lrv\_chart(filtered) & 1,776 & 432 & 24.3 & - & - & - & - \\
lrv\_normal(filtered) & 10,490 & 2,465 & 23.5 & 766 & 7.3 & 766 & 7.3 \\
llavar\_gpt4\_20k & 19,790  & 5,804 & 29.3 & 4,154 & 21.0 & 4,242 & 21.4 \\
mavis\_math\_metagen & 87,348 & 33,022 & 37.8 & 15,426 & 17.7 & 6,431 & 7.4  \\
multihiertt(cauldron) & 7,614 & 2,219 & 29.1 & 208 & 2.7 & 232 & 3.0 \\
MapQA(MathV360K) & 5,225 & 1,248 & 23.9 & 519 & 9.9 & 525 & 10.0 \\
mapqa(cauldron,llava\_format) & 37,412 & 8,689 & 23.2 & 5,507 & 14.7 & 5,256 & 14.0 \\
mavis\_math\_rule\_geo & 99,990 & 11,710 & 11.7 & 3,144 & 3.1 & 1,915 & 1.9 \\
orand\_car\_a & 1,999 & 398 & 19.9 & 111 & 5.6 & 120 & 6.0 \\
PMC-VQA(MathV360K) & 35,948 & 8,031 & 22.3 & 4,084 & 11.4 & 4,044 & 11.2 \\
rendered\_text(cauldron) & 9,995 & 2,963 & 29.6 & - & - & 2,695 & 27.0 \\
robut\_wikisql(cauldron) & 74,984 & 21,053 & 28.1 & - & - & 15,355 & 20.5 \\
raven(cauldron)& 41,995 & 11,709 & 27.9 & 6,407 & 15.3 &7,223 & 17.2 \\
robut\_sqa(cauldron)& 8,509 & 2,269 & 26.7 & - & - & 1,659 & 19.5 \\
robut\_wtq(cauldron,llava\_format)& 38,241 & 8,919 & 23.3 & 5,643 & 14.8 & 5,948 & 15.6 \\
scienceqa(cauldron,llava\_format)& 4,971 & 3,371 & 67.8 & 3,045 & 61.3 & 2,422 & 48.7 \\
sharegpt4o & 57,284 & 19,361 & 33.8 & 1,671 & 2.9 & 6,847 & 12.0 \\
screen2words(cauldron) & 15,725 & 5,139 & 32.7 & 1,536 & 9.8 & 1,466 & 9.3 \\
sharegpt4v(coco)  & 50,017 & 14,985 & 30.0 & 3,074 & 6.1 & 2,482 &  5.0 \\
sharegpt4v(sam)  & 8,990 & 2,682 & 29.8 & 568 & 6.3 & 494 & 5.5 \\
scienceqa(nona\_context)  & 19,208 & 5,729 & 29.8 & 5,139 & 26.8 & 3,855 & 20.1 \\
sharegpt4v(knowledge)   & 1,988& 588 & 29.6 & - & - & 99 & 5.0 \\
st\_vqa(cauldron,llava\_format) & 17,242& 4,880 & 28.3 & - & - & 3,126 & 18.1 \\
sharegpt4v(llava) & 29,990& 7,062 & 23.5 & 1,621 & 5.4 & 1,388 & 4.6 \\
Super-CLEVR(MathV360K)  & 8,642& 2,029& 23.5 & 969 & 11.2 & 997 & 11.5 \\
sroie & 33,616& 4,720& 14.0 & 3,958 & 11.8 & 4,066 & 12.1\\
textcaps  &  21,942 & 6,578& 30.0 & 1,587 & 7.2 & 1,949  & 8.9 \\
textocr(gpt4v)  &  25,104 & 7,487& 29.8 & 1,654 & 6.6 & 1,566 & 6.2\\
tabmwp(cauldron)  & 22,717 & 6,698& 29.5 & 5,983 & 26.3 & 4,568 & 20.1 \\
tallyqa(cauldron,llava\_format)& 98,675 & 27,901& 28.3 & 16,999 & 17.2 & 17,908 & 18.1 \\
TabMWP(MathV360K) & 22,452 & 5,192& 23.1 & - & - & 2,253  & 10.0 \\
tqa(cauldron,llava\_format) & 27,302 & 5,677& 20.8 & 4,743 & 17.4 &  3,538 &13.0 \\
UniGeo(MathV360K) &11,949&2,723& 22.8 & 1,347 &  11.3  & 727& 6.1 \\
ureader\_cap&91,434&16,773 & 18.3 & 3,331 & 3.6 & 4,523 & 4.9 \\
ureader\_ie &17,322&2,177 & 12.6 &  1,078 &  6.2 &  1,114 & 6.4 \\
vistext(cauldron) &9,964&2,981 & 29.9&  1,521  &  15.3 & 1,515 & 15.2 \\
VizWiz(MathV360K) &6,604&1,968 & 29.8& 1,060 & 16.1 &  1,133 & 17.2 \\
visualmrc(cauldron) &3,022&895& 29.6& 793& 26.2 & 771 & 25.5 \\
visual7w(cauldron,llava\_format) &14,361&3,878& 27.0& 3,501 & 24.4 & 3,452 & 24.0 \\
vqarad(cauldron,llava\_format) &308&88& 28.6& 47 & 15.3 & 47 & 15.3 \\
vsr(cauldron,llava\_format)&2,152& 570 & 26.5& 474 & 22.0  & 474  & 22.0 \\
VisualWebInstruct(filtered)&263,584& 55,887 & 21.2& 23,802 & 9.0 & 21,034 & 8.0 \\
vision\_flan(filtered) &186,060& 32,981 & 17.7& 17,876 & 9.6 & 18,169 &  9.8 \\
websight(cauldron)  &9,995& 1,914 & 19.1& 44 & 0.4 & 35 & 0.4 \\
\midrule

Total & 3722953& 639638& 17.2 &301028 & 8.1 & 315228 & 8.47 \\
\bottomrule
\end{longtable}

==> tables/main_re.tex <==
\begin{table*}[t]
\scriptsize
\centering
\newcolumntype{C}{>{\centering\arraybackslash}p{6.5mm}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l*{14}{C}} 
\toprule
\textbf{Model} & Sim & Count & Depth & Jigsaw & ArtStyle & FunCorr & SemCorr & Spatial & Local & VisCorr & MultiV & Refl & Fore & Avg \\

\midrule
\multicolumn{15}{c}{\textbf{Qwen2-VL-7B-Instruct Variants}} \\
\midrule
Qwen2VL-7B & 53.33 & 73.33 & 57.26 & 54.00 & 51.28 & 18.46 & 31.65 & 79.72 & 54.10 & 33.72 & 45.11 & 33.58 & 38.64 & 48.01 \\
Qwen2VL-7B + VTS-V & \cellcolor{green!10}79.26 & \cellcolor{red!5}44.17 & \cellcolor{red!5}53.23 & \cellcolor{green!10}57.05 & \cellcolor{red!5}42.74 & \cellcolor{red!5}12.90 & \cellcolor{red!5}26.67 & \cellcolor{red!5}67.83 & \cellcolor{red!5}49.59 & \cellcolor{red!5}15.72 & \cellcolor{red!5}43.61 & \cellcolor{red!5}32.84 & \cellcolor{red!5}29.55 & 42.70 \\
Ours + VTS-V & \cellcolor{green!10}84.21 & \cellcolor{red!5}63.33 & \cellcolor{green!10}60.48 & \cellcolor{green!10}58.00 & \cellcolor{green!10}76.92 & \cellcolor{green!10}28.35 & \cellcolor{green!10}40.58 & \cellcolor{red!5}60.48 & \cellcolor{green!10}51.64 & \cellcolor{green!10}37.21 & \cellcolor{green!10}47.37 & \cellcolor{green!10}35.82 & \cellcolor{green!10}34.09 & \textbf{52.19} \\
\midrule
\multicolumn{15}{c}{\textbf{LLaMA-3.2-11B-Vision-Instruct Variants}} \\
\midrule
LLaMA3.2-11B & 46.67 & 55.00 & 63.71 & 53.33 & 47.86 & 32.31 & 39.57 & 67.13 & 62.30 & 50.58 & 48.12 & 31.34 & 25.76 & 47.98 \\
LLaMA3.2-11B + VTS-V & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
Ours + VTS-V & \cellcolor{green!10}57.46 & \cellcolor{green!10}56.67 & \cellcolor{green!10}68.55 & \cellcolor{green!10}57.33 & \cellcolor{green!10}55.56 & \cellcolor{green!10}35.43 & \cellcolor{green!10}47.48 & \cellcolor{green!10}69.23 & \cellcolor{red!5}58.20 & \cellcolor{red!5}38.60 & \cellcolor{green!10}52.63 & \cellcolor{green!10}33.58 & \cellcolor{red!5}23.48 & \textbf{50.32} \\
\midrule
\midrule
\multicolumn{15}{c}{\textbf{Qwen2.5-VL-7B-Instruct Variants}} \\
\midrule
Qwen2.5VL-7B & 84.44 & 70.00 & 76.61 & 69.33 & 64.96 & 22.31 & 32.37 & 87.41 & 48.36 & 48.84 & 30.83 & 30.60 & 39.39 & 54.27 \\
Qwen2.5VL-7B + VTS-V & \cellcolor{red!5}82.96 & \cellcolor{red!5}65.00 & \cellcolor{red!5}66.13 & \cellcolor{red!5}59.33 & \cellcolor{red!5}59.83 & \cellcolor{green!10}23.85 & \cellcolor{green!10}36.69 & \cellcolor{red!5}74.83 & \cellcolor{red!5}46.72 & \cellcolor{green!10}58.72 & \cellcolor{green!10}42.86 & \cellcolor{red!5}30.60 & \cellcolor{red!5}38.64 & \cellcolor{red!5}52.78 \\
Ours + VTS-V & \cellcolor{red!5}80.00 & \cellcolor{red!5}65.83 & \cellcolor{red!5}70.97 & \cellcolor{red!5}68.67 & \cellcolor{green!10}67.52 & \cellcolor{green!10}30.00 & \cellcolor{green!10}33.81 & \cellcolor{red!5}86.01 & \cellcolor{green!10}49.18 & \cellcolor{green!10}54.44 & \cellcolor{green!10}55.64 & \cellcolor{green!10}38.06 & \cellcolor{red!5}36.36 & \cellcolor{green!10}\textbf{56.65} \\
\midrule
\multicolumn{15}{c}{\textbf{GPT-4o Variants}} \\
\midrule
GPT-4o & 72.59 & 49.17 & 74.19 & 55.33 & 82.91 & 40.77 & 53.96 & 69.23 & 59.84 & 75.00 & 59.40 & 37.31 & 79.55 & 62.25 \\
GPT-4o + Sketchpad & \cellcolor{green!10}84.20 & \cellcolor{green!10}66.70 & \cellcolor{green!10}83.90 & \cellcolor{green!10}70.70 & \cellcolor{red!5}77.19 & \cellcolor{green!10}42.10 & \cellcolor{green!10}58.30 & \cellcolor{green!10}81.10 & \cellcolor{green!10}65.40 & \cellcolor{green!10}80.80 & \cellcolor{red!5}45.60 & \cellcolor{red!5}33.10 & \cellcolor{red!5}79.00 & 66.78 \\
GPT-4o + CoT & \cellcolor{red!5}63.70 & \cellcolor{green!10}65.00 & \cellcolor{red!5}73.39 & \cellcolor{green!10}62.00 & - & \cellcolor{green!10}57.69 & \cellcolor{green!10}57.55 & \cellcolor{green!10}82.52 & \cellcolor{green!10}60.66 & \cellcolor{green!10}82.56 & \cellcolor{red!5}53.38 & - & - & 65.85 \\
GPT-4o + SoM & \cellcolor{red!5}63.70 & \cellcolor{red!5}43.33 & \cellcolor{red!5}68.55 & \cellcolor{red!5}49.33 & - & \cellcolor{green!10}47.69 & \cellcolor{red!5}52.52 & \cellcolor{green!10}76.22 & \cellcolor{red!5}59.84 & \cellcolor{green!10}83.72 & \cellcolor{red!5}56.40 & - & - & 60.13 \\
GPT-4o + MMFactory & \cellcolor{green!10}75.30 & \cellcolor{green!10}61.70 & \cellcolor{green!10}80.30 & \cellcolor{green!10}75.30 & \cellcolor{green!10}83.00 & \cellcolor{green!10}55.40 & \cellcolor{green!10}58.30 & \cellcolor{green!10}81.80 & \cellcolor{red!5}59.00 & \cellcolor{green!10}85.50 & \cellcolor{green!10}60.20 & \cellcolor{red!5}35.10 & \cellcolor{green!10}84.80 & 68.90 \\
GPT-4o + VTS-V (Ours) & \cellcolor{green!10}85.19 & \cellcolor{green!10}67.50 & \cellcolor{green!10}79.84 & \cellcolor{green!10}75.33 & \cellcolor{red!5}80.34 & \cellcolor{green!10}53.08 & \cellcolor{green!10}56.83 & \cellcolor{green!10}85.31 & \cellcolor{green!10}68.85 & \cellcolor{green!10}82.56 & \cellcolor{red!5}52.63 & \cellcolor{green!10}40.30 & \cellcolor{red!5}71.21 & \textbf{69.15} \\
\bottomrule
\end{tabular}
}
\caption{
\textbf{Model performance on BLINK subtasks.} Columns are reordered to match desired task grouping: Similarity, Count, Depth, Jigsaw, Art, Functionally-Correlated, Semantically-Correlated, Spatial, Local, Visually-Correlated, Multi-view, Reflection, Forensic. \colorbox{green!10}{Improved} and \colorbox{red!5}{degraded} cells are highlighted.
}
\label{tab:blink_results}
\end{table*}
